Dangoron: Network Construction on Large-scale Time Series Data across Sliding Windows

Complex networks represent system dynamics through the interactions of a set of anomalous time series. Consider the problem of computing correlations for highly correlated pairs of time series across sliding windows. Efficiently computing and updating the correlation matrix for user-defined sliding periods and thresholds enables large-scale time series network dynamics analysis. We introduce Dangoron, a framework for effectively identifying highly correlated pairs of time series over sliding windows and computing their exact correlation. By predicting dynamic correlation across sliding windows and pruning unrelated time series, Dangoron is at least an order of magnitude faster than a baseline. Additionally, we propose Tomborg, the first benchmark for the problem of correlation matrix computation.

==> abstract.tex <==
\begin{abstract}
 A complex network represents the complex system by the interactions of a set of anomaly time series. Consider the problem of computing the correlations of the highly correlated pairs of time series over a time window within a sliding window setting. The efficient computation and update of the correlation matrix for the user-defined sliding period and threshold enables the network dynamics analysis on large-scale time series. We present \sys, an algorithm for efficiently finding highly correlated pairs of time series over sliding windows and computing their exact correlation. In TSUBASA, our previous work, by pre-computing simple and low-overhead sketches, we can efficiently compute exact pairwise correlations on arbitrary time windows at query time. Our experiments show that with the same space overhead as a DFT-based approximate solution, TSUBASA has a lower sketching time and is on par with the approximate solution with respect to query time. In this work, we extend the proposed incremental way of updating the correlation matrix to predict the dynamic correlation over sliding windows, skipping the potential unrelated time series on either temporal measurements or spatial ones of the sliding window. We also provide theoretical proof and analysis for the algorithms, showing that \sys can reduce computation complexity. 
\end{abstract}
